An efficient and robust method to estimate halo concentration

We propose an efficient and robust method to estimate the halo concentration based on the first moment of the density distribution, which is $R_1\equiv \int_0^{r_{\rm vir}}4\pi r^3\rho(r)dr/M_{\rm vir}/r_{\rm vir}$. We find that $R_1$ has a monotonic relation with the concentration parameter of the NFW profile, and that a cubic polynomial function can fit the relation with an error $\lesssim 3\%$. Tests on ideal NFW halos show that the conventional NFW profile fitting method and the $V_{\rm max}/V_{\rm vir}$ method produce biased halo concentration estimation by $\approx 10\%$ and $\approx 30\%$, respectively, for halos with 100 particles. In contrast, the systematic error for our $R_1$ method is smaller than $0.5\%$ even for halos containing only 100 particles. Convergence tests on realistic halos in $N$-body simulations show that the NFW profile fitting method underestimates the concentration parameter for halos with $\lesssim 300$ particles by $\gtrsim 20\%$, while the error for the $R_1$ method is $\lesssim 8\%$. We also show other applications of $R_1$, including estimating $V_{\rm max}$ and the Einasto concentration $c_{\rm e}\equiv r_{\rm vir}/r_{-2}$. The calculation of $R_1$ is efficient and robust, and we recommend including it as one of the halo properties in halo catalogs of cosmological simulations.

==> reply.tex <==
Dear Editor-in-chief,

Thank you for forwarding the referee's report on our submission.

We would like to thank the referee for careful reading of the manuscript and
constructive comments. We have addressed the referee's suggestions and
comments, as detailed below. We have highlighted the texts added or revised
based on the referee's suggestion with red faces in the new manuscript.

Yours sincerely,
Kai Wang
On behalf of the co-authors

=========================

* Introduction - "The assembly history of dark matter halos is in strong
correlation to the halo structure" - I think you mean, "The assembly history of
dark matter halos correlates strongly with halo structure"? The English is a
bit clunky here and I suggest it be corrected.

REPLY: we have revised the sentence.

----------------------------------------------------------------
* 2.1 - The description of the HaloFactory package in the appendix is a little
brief, and so some additional details are needed. As far as I can tell,
HaloFactory has not been published and from what I can see it's a fairly
standard python implementation. Figure A1 shows that the code produces stable
halos, which is good. It would help to understand if Eddington's fomula is
solved explicitly, and how the sampling of the distribution function is done.
Is the mass profile tapered and is this accounted for in calculating the
distribution function? I don't think more than a paragraph is required for this.

REPLY: We have added the description of the implementation of the HaloFactory
package at the end of Appendix A.

----------------------------------------------------------------
* 2.2 - I'd recommend that the authors note which codes were used to run the
simulations, as a reminder to the reader. It's also not clear to me what FoF
implementation was used to do the halo finding. SubFind? Was it used in purely
FoF mode (if so, what was the linking length assumed), or was substructure
recovered too?

REPLY:

- We have added more information on the simulations, as quoted below

    - "Dark matter halos are identified using the Friends-of-Friends algorithm
    with a linking length that is 0.2 times the mean inter-particle distance
    (Davis et al. 1985),"

    - "Substructures are identified with the SUBFIND algorithm (Springel et al.
    2001)."

    - "The ELUCID simulation (Wang et al. 2013, 2014, 2016; Tweed et al. 2017)
    is a constrained simulation, run with a memory-optimized version
    of GADGET-2 (Springel et al. 2005) known as L-GADGET, to reconstruct the
    density field and formation history of our local Universe based on the
    Sloan Digital Sky Survey DR7 (York et al. 2000)."

----------------------------------------------------------------
* 4.2 - "While it is not priorly clear" -> "While it is not a priori clear"?

REPLY: Corrected.

----------------------------------------------------------------
* 4.2 - "The second reason is that ... to suppress the unphysical gravity
between the more massive particles" - I think you're trying to say that, for a
given simulation volume, the force softening is larger in lower resolution
runs, and so is a larger fraction of the virial radius in lower mass halos, and
therefore modifies the central mass profile on a larger spatial scale. Is that
correct? If so, can you correct this sentence?

REPLY: Corrected. Here we quote it:

    - "The second reason is that, for a given simulation volume, the force
    softening length is larger in lower resolution runs, and so is a larger
    fraction of the virial radius in lower mass halos, and therefore has a
    larger impact on the central mass profile. This will consequently cause the
    underestimation of halo concentration in the NFW profile fitting method."

----------------------------------------------------------------
* 5 - I think it would help to provide a sentence or two to motivate why you
have looked at the ELUCID simulation. My impression is that the larger volume
and consequently the longer baseline in halo mass allows you to span a larger
dynamic range in concentration, as well as systems in various states of
dynamical relaxation. Of course, your reasoning may differ, but it would
benefit the paper if you could provide some motivation.

REPLY: We have added one sentence to explain our motivation. Here we quote it:

    - "The large volume and relatively high resolution of the ELUCID simulation
    allow us to investigate the mass-concentration relation over a large halo
    mass range."

----------------------------------------------------------------
* 5 - Neto et al. 2007 had combination of criteria to classify halos as relaxed
or unrelaxed - the centre of mass offset (your equation 11), the virial ratio,
and the fraction of halo mass in substructure. Given that you say you use the
Neto et al. criteria but only use the centre of mass offset, can you comment on
why you chose not to use the substructure mass fraction and the virial ratio?
Other authors (e.g. Maccio et al. 2007, Power & Knebe 2012) have looked at the
centre of mass offset and proposed more stringent limits, so it may be worth
commenting on how these different limits may modify your results. I don't think
it will make that much of a different, but commenting on how this, as well as
how using the full Neto et al. criteria, may modify results would be useful to
know fraction and the virial ratio? 

REPLY: We have added our arguments to justify this choice. Here we quote it:

    - "Note that Neto et al. (2007) used two additional conditions to select
    halos in equilibrium. They require that the mass fraction in substructures
    is lower than a threshold value and that the ratio between the kinetic
    energy and the potential energy is lower than a threshold. Here we use only
    the criterion in equation (11), for three reasons. Firstly, as shown in
    Neto et al. (2007), equation (11) alone can select most of the halos in
    equilibrium (see their Figure 2). Secondly, equation (11) is the simplest
    criterion to implement in N-body simulations, whereas the other two
    criteria require either identifying substructures or calculating the
    gravitational potential for each particle. Thirdly, the other two criteria
    suffer from some ambiguities. For instance, the substructure mass fraction
    is subject to the substructure finder used (e.g. van den Bosch & Jiang
    2016) and to the resolution of the simulation (e.g. van den Bosch et al.
    2018). Besides, the exact value of the virial ratio for selecting halos in
    equilibrium is still under debate, as many argued that the surface pressure
    and even the non-spherical shape of halos should be taken into account
    (e.g. Davis et al. 2011; Klypin et al. 2016)."

----------------------------------------------------------------
* 5 - "concentration parameter decreases from 8 to 4 with decreasing mass for
relaxed halos" - do you mean with increasing mass?

REPLY: Corrected.

----------------------------------------------------------------
* Figure 5 - I think it would be worth adding an appendix to comment on the
individual models for the mass concentration relation - what exactly is being
plotted to allow others to reproduce the behaviour in the figure.

REPLY: We have added the following footnote to explain the calculation of these
curves:

    - "All these models are implemented in the \textsc{Colossus} package
    \citep{colossus}, except Zhao+09
    (\url{http://202.127.29.4/dhzhao/mandc.html}) and Correa+15
    (\url{https://www.camilacorrea.com/code/commah/})."

----------------------------------------------------------------
* 5 - "Secondly, the mean logarithmic concentration declines... with a constant
gap of about 0.28 dex" - I am a bit surprised by this. I would expect that
halos at lower masses should be less affected by the cut between relaxed and
unrelaxed, and to see a systematic shift to lower concentrations as we go to
higher masses - and so there should be a gap that increases with mass. Am I
missing something here?

REPLY: This result is consistent with previous results. For instance, from Fig.
7 in Neto+2007, one can see that the difference in the mean concentration for
relaxed and unrelaxed halos is about 0.3 dex for halos with masses around 10^12
solar mass.

----------------------------------------------------------------
* 7 - "However, because of the uncertainty and tedium in their estimations" - I
don't what tedium means in this context. Please clarify.

REPLY: Here we mean that the estimation of halo concentration based on the
conventional fitting method is more time-consuming and more difficult to
implement than our R1 method, as we pointed out in the introduction. Here we
quote it:

    - "Finally, the fitting procedure is relatively time-consuming, making it
    difficult to do for the large number of halos in large cosmological
    simulations. "

----------------------------------------------------------------

